Stand-Up Indulgent Gathering on Rings

We consider a collection of $k \geq 2$ robots that evolve in a ring-shaped network without common orientation, and address a variant of the crash-tolerant gathering problem called the \emph{Stand-Up Indulgent Gathering} (SUIG): given a collection of robots, if no robot crashes, robots have to meet at the same arbitrary location, not known beforehand, in finite time; if one robot or more robots crash on the same location, the remaining correct robots gather at the location of the crashed robots. We aim at characterizing the solvability of the SUIG problem without multiplicity detection capability.

==> geometric-results.tex <==

\begin{theoremEnd}[disc]{lemma}\label{lem:periodic configurations are determined by k/3 consecutive positions}
Let $C$ and $C'$ be two periodic configurations with $k$ occupied positions, and where more than $n/3$ consecutive nodes have the same state (occupied or empty) in both configurations, then $C=C'$.
%\SK{the consecutive occupid nodes may be a sequence of 0,1 (empty and occupied). Is not it correct?}
\end{theoremEnd}
\begin{proofEnd}
Since $n$ is odd, the period of each symmetry is at least $n/3$. So the entire configuration is determined by the state of any $n/3$ consecutive nodes. This implies that $C=C'$.\qed
\end{proofEnd}


\begin{theoremEnd}[disc]{lemma}\label{lem:2 axis of sym => bisector is an axis}
%Let the number of nodes $n$ be odd. AL: as the initial conf is node-edge sym, we know that n is odd 
If a configuration $C$ has two axes of symmetry, then the unique bisector line of these axes passing through a node is also an axis of symmetry.
\end{theoremEnd}
\begin{proofEnd}
Let $q$ be the number of axes of symmetry. Since $n$ is odd, $q$ must be odd as well. Let $L_i$, with $0\leq i < q$ be the axis of symmetry of $C$. We can order the nodes of the ring $u_0, u_1, \ldots u_{n-1}$ so that $L_0$ contains $u_0$ and, more generally $L_i$ contains $u_{in/q}$. Now we show that the bisector line of any pair of axes $L_i$ and $L_j$, with $i\neq j$, is another axis.

If $i+j$ is even, then, clearly, $L_{\frac{i+j}{2}}$ is the line bisector of $L_i$ and $L_j$. Otherwise, one can see that the line bisector is $L_{q'}$, with $q'\equiv \frac{i+j+q}{2} \mod q$.\qed
\end{proofEnd}

We know that if a secondary robot that is ordered to move is crashed, the resulting configuration is quasi-node-edge-symmetric and quasi-periodic. 
The next lemma states that in this case there exists no other quasi-axis of symmetry.
\begin{theoremEnd}[disc]{lemma}\label{lem:even quasi-axis is unique}
If a configuration with more than 3 occupied nodes has a $\{r_1, r_1'\}$-quasi-axis of symmetry with even gap distance, and is $r_1$-quasi-periodic, then it does not have another quasi-axis (regardless of its parity).
\end{theoremEnd}
\begin{proofEnd}
Let $C$ be a configuration that is $\{r_1, r_1'\}$-quasi-symmetric with an even gap distance. We know that this also implies that $C\setminus\{r_1\}\cup\{\bar{r_1'}\}$ is periodic with period $p\geq 3$ (that is odd, because $n$ is odd) and is symmetric, with axis $L_1$, so the string of node states is $S=(a_{m}a_{m-1}\ldots a_2a_1a_0 a_1a_2\ldots a_{m-1} a_m)^{n/p}$, with $m = (p-1)/2$. Assume for the sake of contradiction that there is another $\{r_2, r_2'\}$-quasi-axis $L_2$. The gap distance associated with $L_2$ is smaller than $n/3$, otherwise, let $P$ be the path joining $r_2$ and $r_2'$ of length the gap distance. Either, (i) there is no other robot on $P$, so there are at most three occupied nodes (recall that by moving one robot the configuration is periodic), or (ii) there is one robot on $P$, or (iii) $P$ consists only of occupied nodes so that the whole configuration as well. Each case implies a contradiction.
So there are two paths $P_1$ and $P_2$ that are disjoint, symmetric with respect to $L_2$ and have length $p$. $r_1$ and $\bar{r_1}'$ cannot be on different sides of $L_2$ (because they have different state so they cannot be symmetric -- recall that they are adjacent) so lets say $P_1$ contains $r_1$ and $\bar{r_1}'$.
Since $P_1$, resp. $P_2$, is of length at least $p$, it contains a full copy of the periodic string of states $S$ (up to cyclic permutation). 
%Let $i_1$ the index in the string that correspond to the state of the node at $r_1$. 
Moreover, by assumption, $r_1$ should not be there for the configuration to be periodic so that, in the string of state in $P_1$ is actually cyclic  permutation $\sigma_1$ of $S'= a_m a_{m-1}\ldots \lnot a_{i_1+1} \lnot a_{i_1} \ldots a_2a_1a_0 a_1\ldots a_{m-1} a_m$ for some $i_1\in [0, m]$, while in $P_2$ it is a cyclic permutation $\sigma_2$ of $S$. So we have $\sigma_1S' = \sigma_2S$ (because $P_1$ and $P_2$ are symmetric with respect to $L_2$). This implies that $\lnot a_{i_1} = a_{i_2}$ and also that $a_{i_2} = a_{i_1}$, which is a contradiction. \qed
% (recall that $a_{i_1}$ appears two times in the string $S$), which is a contradiction. If $i_1 = 0$, then $\lnot a_{0} = a_{i_2}$ but we also have $a_{0} = a_{i_2}$
%Maybe I should rewrite this with better notation, maybe by using indexes of nodes instead of states, and with a function returning the state, idk.
\end{proofEnd}

\vspace{-2mm}
\begin{theoremEnd}[disc]{lemma}
\label{lem:initial config remains non-periodic with crash}
Let $C\in \NE(k) \setminus P$ with $k>3$ occupied nodes, and $C\oneRound C'$, then $C'\not\in\Periodic$, even if there exists a crashed robot.
\end{theoremEnd}
\begin{proofEnd}
The proof is similar to the proof of Lemma~\ref{lem:even quasi-axis is unique}. Indeed, $C'$ is quasi-periodic and has an axis of symmetry. \qed
\end{proofEnd}
\vspace{-2mm}
\begin{theoremEnd}[disc]{lemma}
Let $C\in \QNE(k)\setminus \NE(k) \setminus P$ with $k>3$. If all quasi-axes of $C$ have odd gap distances, then, either
\begin{itemize}
    \item all quasi-axes have the same orientation, or
    \item there are exactly two quasi-axes with opposite orientation.
\end{itemize}
\end{theoremEnd}
%\begin{lemma}
%If a configuration $C$ is $\{r_1, r_1'\}$-quasi-node-edge symmetric and $\{r_2, r_2'\}$-quasi-node-edge symmetric, with $\{r_1, r_1'\}\neq \{r_2, r_2'\}$, with gap distances having the same parity, then $C$ is node-edge symmetric or the direction associated with each quasi-axis is the same.
%\end{lemma}
\begin{proofEnd}
Consider two arbitrary quasi-axes of $C$, $\{r_1, r_1'\}$-quasi-axis $L_1$ and  $\{r_2, r_2'\}$-quasi-axis $L_2$. 
Recall the notations such that $C\setminus\{r_1\}\cup\{\bar{r_1'}\}$ (resp. $C\setminus\{r_2\}\cup\{\bar{r_2'}\}$) are node-edge symmetric with respect to $L_1$ (resp. $L_2$). In particular, we have that $L_1\neq L_2$. 

Let $d_1$ be the gap distance of $\{r_1, r_1'\}$ and $d_2$ be the gap distance of $\{r_2, r_2'\}$.
By assumption, $d_1$ and $d_2$ are odd.

Without loss of generality, we assume $r_1$ is the leading robot among $\{r_1, r_1'\}$.
From now, we choose for the orientation of the rotations the orientation associated $\{r_1, r_1'\}$, i.e., such that $r_1 = \rot(d_1)(r_1')$ (in the following figures, we use the counterclockwise direction).

Let $s_1$ (resp. $s_2$) be the symmetry transformation with respect to $L_1$ (resp. $L_2$). For any nodes $u$ and $v$, we write $u \apps{1} v$ when $v = s_1(u)$.
Consider the following longest sequence of occupied nodes $u_0, u_1, u_2, \ldots, u_m$ such that
\begin{equation}\label{eq:seq from r1 to r2}
r_1 = u_0 \apps{2} u_1 \apps{1} u_2\apps{2} \ldots \apps{i} u_m
\end{equation}
We have to consider two cases depending on the value of $i$, either the last symmetry is $s_1$ or $s_2$.\\
\textbf{Case 1: $i=1$.}
In this case, $s_2(u_m)$ is not a robot (otherwise the sequence is not maximal). The only robots that do not have symmetric robots with respect to $L_2$ are $r_2$ and $r_2'$, so $u_m$ is either $r_2$ or $r_2'$. Without loss of generality (since both robots are interchangeable in the definition) assume $u_m = r_2$.

Similarly, there exists another sequence 
\[
r_1' \apps{2} u_1' \apps{1} u_2'\apps{2} \ldots \apps{i} u'_{m'}
\]
where $u'_{m'} = r_2'$.

We consider four sub-cases (recall that we assumed w.l.o.g. that $r_1 = \rot(d_1)(r_1')$, otherwise the results is obtained by symmetry).


\input{../Figures/case1a-1b}


\textbf{Case $1.a$:} $r_2' = \rot(d_2)(r_2)$ and $r_2'$ is the leading robot (see Figure~\ref{fig:case 1.a}).

In this case, the orientation of the two quasi-axes are the same.


\textbf{Case $1.b$:} $r_2 = \rot(d_2)(r_2')$ and $r_2$ is the leading robot (see Figure~\ref{fig:case 1.b}).%; or $r_1 = \rot(x+1)(l_1)$ and $r_2 = \rot(x+1)(l_2)$.

In this case, the orientation of the two quasi-axis are the same.

%
%    CASE 1.c
% 
\textbf{Case $1.c$:} $r_2 = \rot(d_2)(r_2')$ and $r_2'$ is the leading robot (see Figure~\ref{fig:case 1.c}).

In this case, we need a more careful analyze of the situation. We know that applying two axial symmetries is equivalent to applying a rotation whose angle is two times the angle formed by the two axes of symmetry (in more details, the angle of the rotation associated with the composition of axial symmetry of axis $L_2$ followed by the axial symmetry of axis $L_1$ is two times the angle of the rotation mapping $L_2$ to $L_1$).
Here, let $\rho$ be the angle of the rotation $s_1\circ s_2$. In other words, $\rho$ is such that $\rot(\rho/2)(l_2)=l_1$, where $l_1$ (resp. $l_2$) is the target node associated with $L_1$ (resp. $L_2$).

\input{../Figures/case1c-1d}

From (\ref{eq:seq from r1 to r2}) we deduce that $r_2 = \rot(\rho m/2)(r_1)$. Similarly 
\begin{equation}\label{eq:case1c eq1}
    r_2' = \rot(\rho m'/2)(r_1').
\end{equation}
Moreover, in this case we have 
\begin{align*}
\left.\begin{array}{rl}
r_1 &= \rot(d_1)(r_1')\\
r_2 &= \rot(\rho m/2)(r_1)\\
r_2' &= \rot(-d_2)(r_2)\\
\end{array}\right\}
\Rightarrow r_2' = %\rot(-2x-1 + \rho m/2 + 2x+1)(r_1') =
\rot(\rho m/2+d_1-d_2)(r_1').
\end{align*}
With Equation~(\ref{eq:case1c eq1}), this implies
\[
\rot\left(\rho\frac{m}{2}+d_1-d_2\right) = \rot\left(\rho\frac{m'}{2}\right)
\]
so that 
\begin{equation}\label{eq:case1c:eq2}
\rot(\rho\frac{m - m'}{2}) = \rot(d_2-d_1).
\end{equation}

Another interesting observation is to see that, since $\overline{r_1} = s_1(r_1)$ and $\overline{r_2} = s_2(r_2)$, we in fact have $\overline{r_2} = \rot\left(-\rho\left(\frac{m}{2} + 1\right)\right)(\overline{r_1})$ (it is like extending the sequence $(u_i)_i$ one point before and one after, and the sequence of symmetries now starts with $s_1$ instead of $s_2$, so the rotation is opposite). And since $\overline{r_1} = \rot(1)(r_1')$ and $\overline{r_2} = \rot(1)(r_2')$, then we have 
\[
r_2' = \rot\left( -\rho\left(\frac{m}{2} + 1\right) + 2\right)(r_1')
\]
with Equation~(\ref{eq:case1c eq1}) we obtain
\begin{equation}\label{eq:case1c:(m+m')/2+1}
\rot\left(\rho\left(\frac{m+m'}{2} + 1\right)\right)  = \rot\left(2\right)
\end{equation}

We now show that $d_2 = d_1$ and $m=m'$. First, assume for the sake of contradiction that $d_1 \neq d_2$ (then clearly $m\neq m'$, otherwise $\rot\left(\rho\frac{m - m'}{2}\right) = \rot(0) = \rot(d_2-d_1)$ is a contradiction).
Assume that $d_1 < d_2$ and $m>m'$ (the other cases are proved in a similar way).
If $(m-m')/2$ is even, Equation~(\ref{eq:case1c:eq2}) implies $\rot(\rho\frac{m - m'}{4}) = \rot\left(\frac{d_2-d_1}{2}\right)$. So we have
\[
u_{m-2\frac{m-m'}{4}} = \rot\left(-\rho\left(\frac{m-m'}{4}\right)\right)(r_2)= \rot\left(-\frac{d_2-d_1}{2}\right)(r_2).
\]
so the robot at $u_{m-2\frac{m-m'}{4}}$ is between $r_2'$ and $r_2$, at distance $0 < \frac{d_2-d_1}{2} < d_2$ from $r_2$. But a robot can be between $r_2$ and $r_2'$ only if it is on the quasi-axis $L_2$ (it is the target node), so at distance $(d_2 + 1)/2$ from $r_2$, which implies that $d_1= - 1$, which is a contradiction. 
%If $(m-m')/2$ is odd, so is  $(m+m')/2$ (because $m'$ is even), so $(m+m')/2 + 1$ is even. 
If $(m-m')/2$ is odd, then $(m+m')/2$ is also odd (because $(m+m')/2 = (m-m')/2+m'$ and $m'$ is even). Thus, $(m+m')/2 + 1$ is even.
However, we know that $\rot\left(-\rho\left(\frac{m+m'}{2} + 1\right)\right)=\rot(2)$ (Equation~\ref{eq:case1c:(m+m')/2+1}), so that, by dividing by two, $\rot\left(-\rho\left(\frac{\frac{m' + m}{2} + 1}{2}\right)\right)=rot(1)$. Since either $m/2$ or $m'/2$ is greater than $a = \frac{\frac{m' + m}{2} + 1}{2}$ we obtain a contradiction: either robot $u_{m - 2a}=\rot(-1)(r_2)$ is a robot located at $\bar{r_2'}$ (which should be empty) or robot $u_{2a}' = \rot(1)(r_1')$ is a robot located at $\bar{r_1}$.

Hence, we know that $m = m'$ and $d_1=d_2$. This implies that $r_1$ and $r_2'$ are symmetric with respect to the line $L_3$, bisector of $L_1$ and $L_2$. Similarly, $s_2(r_1)$ is the symmetric of $s_1(r_2')$ with respect to $L_3$, $s_1(s_2(r_1))$ is the symmetric of $s_2(s_1(r_2'))$, etc...
 The two sets of robots $\{u_i\}_{0\leq i\leq m}$ and $\{u_i'\}_{0\leq i\leq m}$ are symmetric with respect to $L_3$.

If some robots are not in this sets, i.e., $R' = R\setminus \left(\{u_i\}_{0\leq i\leq m} \cup \{u_i'\}_{0\leq i\leq m}\right)\neq \emptyset$, then both $L_1$ and $L_2$ are axes of symmetry of $R'$ (because the configuration is quasi-symmetric for $L_1$ and $L_2$), hence, by Lemma~\ref{lem:2 axis of sym => bisector is an axis}, $L_3$ is also an axis of symmetry of $R'$.
Hence, the whole configuration is node-edge-symmetric with respect to $L_3$, a contradiction.

%
%    CASE 1.d
% 
\textbf{Case $1.d$:} $r_2' = \rot(d_2)(r_2)$ and $r_2$ is the leading robot (see Figure~\ref{fig:case 1.d}).

We first show that $\frac{m'+m}{2}$ is even. 
We have, using the same notation as in case $1.c$, 
\begin{equation}\label{case1.c two equations}
\begin{array}{l}
\rot(d_1-1 + \rho m + d_2-1) = \rot(-\rho) \\
\rot(1-d_1 + \rho m' + 1-d_2) = \rot(-\rho)
\end{array}
\end{equation}
and we obtain by addition
\[
\rot(\rho ((m' + m) + 2)) = \rot(0).
\]
Since $n$ is odd and $m'+m$ is even, we have
\[
\rot\left(\rho \left(\frac{m' + m}{2} + 1\right)\right) = \rot(0)
\]
If we assume for the sake of contradiction that $\frac{m' + m}{2} + 1$ is even, then,
\[
\rot\left(\rho \left(\frac{\frac{m' + m}{2} + 1}{2}\right)\right) = \rot(0)
\]
 and since either $m/2$ or $m'/2$ is greater than $a = \frac{\frac{m' + m}{2} + 1}{2}$, we obtain a contradiction ($u_{2a}$ is collocated with $r_1$ or $u_{2a}'$ is collocated with $r_1'$, and this would create a cycle in the sequence $u_0, u_1,\ldots$, which is not possible).

So we know that $\frac{m' + m}{2}$ is even. We now show that $d_1 = d_2$. We can subtract and divide by 2 the two Equations~(\ref{case1.c two equations}) to obtain
\[
\rot\left(\rho \left(\frac{m' - m}{2}\right)\right) = \rot(d_2+d_1+2)
\]
%\begin{align*}
%\rot\left(\rho \left(m' - m\right)\right) = \rot\left(2d_2+2d_1+4\right)
%\end{align*}
Since $\frac{m' - m}{2}$ is even and $d_2+d_1$ is also even (recall that $d_1$ and $d_2$ are odd), we can again divide by 2:
\begin{align*}
    \rot\left(\rho \left(\frac{m' - m}{4}\right)\right) = \rot\left(\frac{d_2+d_1}{2}+1\right)
\end{align*}
If, by contradiction, $d_1\neq d_2$, then either $d_1$ or $d_2$ is at most $\frac{d_2+d_1}{2}+1$.  This implies that a robot in the sequence $(u_i)_i$ or $(u_i')_i$ is between $r_1$ and $r_1'$ or between $r_2$ and $r_2'$. Assume that $m' > m$ and $d_1\leq \frac{d_2+d_1}{2}+1$ (the other cases are done in a similar way). Then the robot at $u_{2\frac{m'-m}{4}}'$ is between $r_1$ and $r_1'$,  at distance $\frac{d_2+d_1}{2}+1$ from $r_1'$. The only robot that might be in between those robots is a robot that is on the quasi-axis (the target node), so at distance $\frac{d_1 + 1}{2}$ from $r_1'$, but $\frac{d_2+d_1}{2}+1>\frac{d_1 + 1}{2}$ so this is not possible.
%QB: maybe I have to add detail for the above affirmation

So we know $d_1=d_2$ and this implies that $r_1$ and $r_2$ are symmetric with respect to $L_3$, the line bisector of $L_1$ and $L_2$. In turn, $s_2(r_1)$ and $s_1(r_2)$ are also symmetric with respect to $L_3$. $s_1(s_2(r_1))$ and $s_2(s_1(r_2))$ as well and so on. The same thing is true between $r_1'$ and $r_2'$, so $L_3$ is an axis of symmetry of the set of robots $R_{seq} = \{r_1, r_1', u_1, u_1', \ldots, u_m, u_m'\}$.

If some robots are not in this set i.e., $R' = R\setminus R_{seq}\neq \emptyset$, then both $L_1$ and $L_2$ are axes of symmetry of $R'$ (because the configuration is quasi-symmetric for $L_1$ and $L_2$), hence, by Lemma~\ref{lem:2 axis of sym => bisector is an axis}, $L_3$ is also an axis of symmetry of $R'$.

Hence, the whole configuration is node-edge-symmetric with respect to $L_3$.\\
%\textbf{Case $1.b$:} $r_1 = \rot(x+1)(l_1)$ and $r_2 = \rot(-x-1)(l_2)$. The proof is the same as the previous case.
%
%    CASE 2
% 
\textbf{Case 2: $i=2$.}
Then $u_m = r_1'$. Again, since $s_1\circ s_2 = \rot(\rho)$, we have that 
\[
r_1 \apprho{} u_2 \apprho{} u_4 \apprho{} \ldots  \apprho{} u_{m-1} \apprho{} \bar{r_1'}
\]
Where $u_{m-1} \apprho{} \bar{r_1'}$ because $u_m \apps{1} \bar{r_1'}$. So we have $\bar{r_1'} = \rot(\rho m/2)(r_1)$.
Since $r_1$ and $\bar{r_1'}$ are adjacent (more precisely, we assumed w.l.o.g that $\bar{r_1'} = \rot(1)(r_1)$) then $\rho m/2 \equiv 1 \mod n$ and this implies that $\rho$ and $n$ are coprime. Hence, $m$ is the smallest integer such that $\rho m/2 \equiv 1 \mod n$ (otherwise each node contains a robot). 

We can do the same starting from $r_2$, but this time the sequence starts with $s_1$:
\[
r_2 \apps{1} u_1' \apps{2} u_2'\apps{1} \ldots \apps{1} u_k'
\]
where $u_k'=r_2'$, hence we have
\[
r_2 \apprho{-1} u_2' \apprho{-1} u_4' \apprho{-1} \ldots  \apprho{-1} u_{m'-1}'
\apprho{-1} \bar{r_2'}
\]
 Using the same argument as previously, we know that $m' = m$. Thus, $r_2 = \rot(\rho m/2)(\bar{r_2'})$, but since $\rot(\rho m/2)=\rot(1)$, we have $r_2 = \rot(1)(\bar{r_2'})$, which implies that the two quasi-axis have opposite orientations, as depicted in Figure~\ref{fig:case 2 example}.%, as depicted in Figure~\ref{fig:case 2} (and cannot be as depicted in Figure~\ref{fig:case 2'})
 % QB: the following is not true anymore (d_1 != d_2), and $r_1$ and $r_2$ are symmetric with respect to the line $L_3$, bisector of $L_1$ and $L_2$.
 %Similarly, $s_2(r_1)$ is the symmetric of $s_1(r_2)$ with respect to $L_3$, $s_1(s_2(r_1))$ is the symmetric of $s_2(s_1(r_2))$, etc... 
% The two sets of robots $\{u_i\}_{0\leq i\leq m}$ and $\{u_i'\}_{0\leq i\leq m}$ are symmetric with respect to $L_3$.
%If some robots are not in this sets i.e., $R' = R\setminus \left(\{u_i\}_{0\leq i\leq m} \cup \{u_i'\}_{0\leq i\leq m}\right)\neq \emptyset$, then both $L_1$ and $L_2$ are axes of symmetry of $R'$ (because the configuration is quasi-symmetric for $L_1$ and $L_2$), hence, by Lemma~\ref{lem:2 axis of sym => bisector is an axis}, $L_3$ is also an axis of symmetry of $R'$.
%So the whole configuration is symmetric with respect to $L_3$.

So, in this case, it is possible to have two quasi-axis with opposite orientations. We now prove that the configuration cannot have a third quasi-axis. Indeed, if the configuration has a $\{r_3, r_3'\}$-quasi-axis $L_3$, then it has an orientation opposite to either $\{r_1,r_1'\}$ or $\{r_2,r_2'\}$. Assume w.l.o.g that the orientation of $\{r_3, r_3'\}$ is opposite with $\{r_1, r_1'\}$. This means that we can do the same reasoning between these two quasi-axis as between $\{r_1,r_1'\}$ and $\{r_2,r_2'\}$, using the $s_3$ symmetry of axis $L_3$ instead of the $s_2$ symmetry. In this reasoning, we have two sequences of robots:
\begin{align*}
r_1 = v_0 \apps{3} v_1 \apps{1} v_2\apps{3} \ldots \apps{i} v_{m_{1,3}}\\
r_1' = v'_0 \apps{3} v'_1 \apps{1} v'_2\apps{3} \ldots \apps{i} v'_{m'_{1,3}}
\end{align*}
However, only {\bf Case 2} is possible (because we saw that if {\bf Case 1} applies, the two quasi-axis have the same orientation). Hence, by denoting $\rho_{1,3} = s_1\circ s_3$, we have
\begin{align*}
    \bar{r_1'} &= \rot(\rho_{1,3} m_{1,3}/2)(r_1)\\
    r_3 &= \rot(\rho_{1,3} m_{1,3}/2)(\bar{r_3'})
\end{align*}
and $m_{1,3}$ is the smallest integer such that $\rho_{1,3} m_{1,3}/2 \equiv 1 \mod n$. One can see that at least one robot is either $(i)$ in the sequence $(u_i)_i\cup(u'_i)_i$ but not in $(v_i)_i\cup(v'_i)_i$ or the contrary $(ii)$ in the sequence $(v_i)_i\cup(v'_i)_i$ but not in $(u_i)_i\cup(u'_i)_i$. Indeed, otherwise $m_{1,3} = m$, which implies $\rho = \rho_{1,3}$, which implies $L_2 = L_3$, a contradiction.
Assume case $(i)$ without loss of generality. So a robot $r$ is not $(v_i)_i\cup(v'_i)_i$. When we apply sequentially $\rho_{1,3}$, we never obtain a robot in $(v_i)_i\cup(v'_i)_i$, so the set of robot $(\rho_{1,3}^i(r))_i$ is finite and periodic. However, since $\rho_{1,3}$ and $n$ are coprime, this is not possible. So, there is at most two quasi-axis of symmetry with opposite orientation. \qed


\begin{figure}
    \centering
\begin{tikzpicture}
\tikzstyle{robot}=[circle,fill=black!100,inner sep=0.05cm]
  
\def\n{25}
\def\radius{2.4cm}
\confRing

\confAxis[dashed]{0}{-4}{20}
\confAxis[dashed]{6}{-4}{20}

\confRobot[]{1}
\confRobot[red]{-2}
\confRobot[]{4}
\confRobot[]{-4}

\confRobot[red]{9}
\confRobot[]{-9}

\confRobot[]{11}
\confRobot[]{-11}

\end{tikzpicture} 
    \caption{Case 2: a configuration with two quasi-axis with opposite orientations. The crashed robot is one of the red robots.}
    \label{fig:case 2 example}
\end{figure}

\end{proofEnd}
